Grounding Task Assistance with Multimodal Cues from a Single Demonstration

A person's demonstration often serves as a key reference for others learning the same task. However, RGB video, the dominant medium for representing these demonstrations, often fails to capture fine-grained contextual cues such as intent, safety-critical environmental factors, and subtle preferences embedded in human behavior. This sensory gap fundamentally limits the ability of Vision Language Models (VLMs) to reason about why actions occur and how they should adapt to individual users. To address this, we introduce MICA (Multimodal Interactive Contextualized Assistance), a framework that improves conversational agents for task assistance by integrating eye gaze and speech cues. MICA segments demonstrations into meaningful sub-tasks and extracts keyframes and captions that capture fine-grained intent and user-specific cues, enabling richer contextual grounding for visual question answering. Evaluations on questions derived from real-time chat-assisted task replication show that multimodal cues significantly improve response quality over frame-based retrieval. Notably, gaze cues alone achieves 93% of speech performance, and their combination yields the highest accuracy. Task type determines the effectiveness of implicit (gaze) vs. explicit (speech) cues, underscoring the need for adaptable multimodal models. These results highlight the limitations of frame-based context and demonstrate the value of multimodal signals for real-world AI task assistance.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/rebuttal_v5.tex <==
We thank the AC and the external reviewers (R1, R2, R3) for their detailed feedback. We appreciate the recognition of our system’s potential and the thoughtful suggestions to strengthen our clarity, evaluation, and novelty claims. Below, we address the primary concerns raised by reviewers.
 
MOTIVATION & USE CASES (R2, R3)
R2, R3 suggested that the original motivation and use cases could be clarified. We have revised the introduction to provide clearer examples and scenarios that ground our approach in everyday tasks. We encourage the reviewers to read the updated introduction, which now highlights real-world contexts and clarifies how these tasks benefit from our multimodal, demonstration-based approach.
 
EVALUATION APPROACH & REALISM (R2, R3)
Reviewers expressed concerns that the evaluation felt not sufficiently generalizable. Our approach balances controlled, systematic evaluation with the incorporation of realistic tasks. We employed a controlled lab environment to ensure consistency and mitigate confounders, while still varying objects, locations, and task types (organizing, shopping, morning routines) to ensure personalization and natural task execution. Although a lab study cannot capture all the complexities of the real world, we have supplemented our revisions with additional full-length videos demonstrating the system’s utility in a real apartment. This is included in the newly provided video figure with cleaning (demo at 6:15; real-time at 16:24) and breakfast preparation (demo at 26:42; real-time at 30:40).
 
PRESENTATION & CLARITY (R2)
R2 noted that the presentation could be clearer, especially for first-time readers. In response, we have reorganized the introduction, made explicit connections between related work and our contributions, corrected missing citations, and refined the results with bolded callouts of important findings. We also split Figure 1 into smaller visuals and added a teaser figure. These changes aim to improve readability and comprehension.
 
NOVELTY & RELATION TO PRIOR WORK (R1)
R1 requested clearer articulation of our novelty compared to prior work. We emphasize in the revised introduction and related work sections that our system integrates both implicit (gaze, gestures) and explicit (speech) cues in a single demonstration, without task-specific pretraining. This contrasts with prior efforts that rely heavily on visual retrieval alone or task/domain-specific models and systems. Unlike AR-based authoring frameworks, our approach generalizes across tasks without requiring domain-specific engineering. We highlight that our approach generalizes across a wide range of tasks and that our analysis of how gaze and speech interact to produce reliable assistance is novel. We have expanded citations, improved figures, and encourage reviewers to see Section 6 for clarified results.
 
QUALITATIVE FEEDBACK & PARTICIPANT INSIGHTS (R3)
R3 requested more qualitative feedback. In Section 6.3, we provide extensive behavioral coding of participant utterances, revealing how speech patterns differed by task type (e.g., more structured directives for organizing tasks, more preference-based commentary for shopping, and more procedural queries for cooking). This approach allowed us to gain meaningful insights into participants' interactions with our system, without relying on self-reported measures.
 
VERBAL ANNOTATIONS & MULTIMODALITY (R2)
R2 inquired the practicality of verbal annotations. In Section 6.2, our analysis shows a significant interaction between task type and condition, indicating that while gaze excels in some scenarios, speech improves others. Together, these two modalities offer richer, more personalized assistance, demonstrating that verbal annotations are often not redundant but play a crucial complementary role for improving specificity and clarity of user’s desired intent.

BASELINE COMPARISONS & FRAME SELECTION (R1)
R1 suggested that modern VLMs might perform well without demonstration videos. To clarify, we compare against a zero-shot baseline that lacks these demonstrations (Section 7, 7.1, Figure 8). Its significantly lower performance (30.47% no demo (zero shot) vs. 63.2% for our approach - MICA gaze + speech) indicates the necessity of contextual information from the demonstration. Concerns about the selection of key frames among unsampled frames are addressed in Appx. S5, Fig S1-S4. We have also included additional retrieval analysis in Appx. S1.2 and S1.4. We added more discussion of Ego4D and Ego-Exo4D in related works Section 2.3.
 
Note to Reviewers: We identified a mistake in our evaluation: a ground truth task description was inadvertently provided in one experiment for the gaze condition. Correcting this resulted in a 3.2% reduction in performance, making the difference between gaze and speech conditions statistically significant. Our conclusions remain the same when using a ground truth task description. The gaze condition still outperforms baseline methods. This correction is now reflected in the revised manuscript (see Section 6.1, conclusions 3 and 4).
